On Wasserstein Reinforcement Learning and the Fokker-Planck equation

Policy gradients methods often achieve better performance when the change in policy is limited to a small Kullback-Leibler divergence. We derive policy gradients where the change in policy is limited to a small Wasserstein distance (or trust region). This is done in the discrete and continuous multi-armed bandit settings with entropy regularisation. We show that in the small steps limit with respect to the Wasserstein distance $W_2$, policy dynamics are governed by the Fokker-Planck (heat) equation, following the Jordan-Kinderlehrer-Otto result. This means that policies undergo diffusion and advection, concentrating near actions with high reward. This helps elucidate the nature of convergence in the probability matching setup, and provides justification for empirical practices such as Gaussian policy priors and additive gradient noise.

==> comments.tex <==
The fact that optimizing approximate KL divergences leads to exponential families is not new. A great number of statistical inference methods can be seen as instances of this general result : there is convex duality between maximum entropy and maximum likelihood estimation.


(regularising max likelihood by approximate moment matching enables us to prevent overfitting)

Add on Wasserstein bias / Cramer
Add on W_2 rather than W_1 : Kantorovich potential math

3.3 : Tilting takes away from the linear part, turns the functional into pure entropy and the transport PDE into a pure PDE `: the SDE view of this is just an evolution strategy.
In fact 3.3 opens the door to a comparison with boosting in an exp loss context : policy boosting.

Add to the conclusion that extension to various other Bregman divergences and to the multistep case are considered.

'Any Bregman or Cziszar divergence satisfies convex duality ; the KL is the only one that is both'

In conclusion : link the W2 entropic regularization term to a disentanglement term ala InfoGAN ?

3.5 $\pi = \diag(a) \xi \diag(b)$ $a \in \mathbb{R}^q$ $b \in 'mathbb{R}^q$
$\xi = e^{-c/ \ gamma}$

'the optimal \emph{coupling} is a diagonal scaling of the ground cost's Gibbs kernel'

